Towards Understanding Limitations of Pixel Discretization Against Adversarial Attacks

Wide adoption of artificial neural networks in various domains has led to an increasing interest in defending adversarial attacks against them. Preprocessing defense methods such as pixel discretization are particularly attractive in practice due to their simplicity, low computational overhead, and applicability to various systems. It is observed that such methods work well on simple datasets like MNIST, but break on more complicated ones like ImageNet under recently proposed strong white-box attacks. To understand the conditions for success and potentials for improvement, we study the pixel discretization defense method, including more sophisticated variants that take into account the properties of the dataset being discretized. Our results again show poor resistance against the strong attacks. We analyze our results in a theoretical framework and offer strong evidence that pixel discretization is unlikely to work on all but the simplest of the datasets. Furthermore, our arguments present insights why some other preprocessing defenses may be insecure.

==> Makefile <==
### Makefile --- 

TARGETS = paper

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -bibtex -c # clean up regeneratable files

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls


==> ideal.tex <==
To garner additional insights, we propose and analyze an idealized
model under which we can precisely analyze when our method can improve
adversarial robustness. Roughly speaking, our results suggest the
following: Suppose that data is good in the sense that it can be
``generated'' using some ``ground-truth'' codewords that are
sufficiently separated; then, as long as we can find a
$\nu$-approximation for the ground truth and we have a base model $F$
that is robust with respect to the $\nu$-approximation, it follows
$F(T(\cdot))$ is immune to any adversarial attack with budget $\epsilon \le 5\nu$,
thus providing a boost of adversarial robustness. We now present details.

\noindent\textbf{Idealized generative model of images.} 
Suppose each pixel $\bfx[i]$ is $3$ dimensional vector of discrete values in $[K]={1,2,\ldots, K}$.
Suppose there is a set of ground-truth codes $\mathcal{C}^*=\{c^*_1, \ldots, c^*_k\}$,
where the codes are well separated so that $\|c^*_i - c^*_j\| \ge \Gamma$ for some large $\Gamma$.
Each image is generated by first generating a skeleton image $\mathbf{u}$ where each pixel is a code,
and then adding noise to the skeleton. We do not make assumptions about generating the label $y$. Formally,
\begin{enumerate}
\item $\mathbf{u}$ is generated from some distribution over $(\mathcal{C}^*)^d$,
  where the marginal distribution satisfies $P(c^*_i) = 1/k,\forall i$.
\item $\bfx[i] = \mathbf{u}[i] + \zeta$, where $\zeta$ takes valid discrete values so that $\bfx[i] \in [K]^3$, and
  \begin{align*}
    \|\zeta\| \le \Gamma/8, ~\text{and}~ \text{Pr}[\|\zeta\| = t] = \alpha \exp(-t^2/\sigma^2)
  \end{align*}
  where $t\le \Gamma/8$ takes valid discrete values, $\sigma$ is a parameter,
  and $\alpha$ is a normalization factor. 
\end{enumerate}

\noindent\textbf{Quantifying robustness.}  We now prove our main
theoretical result in the idealized model.  We say that a set of
codewords $\{c_1, \dots, c_k\}$ is a \emph{$\nu$-approximation} of
$\mathcal{C}^*$ if for any $i$, $\| c_i - c_i^*\| \le \nu$. For the
above generative model, one can show that the codewords found by
Algorithm~\ref{alg:find} are $\nu$-approximation of the ground truth
$\mathcal{C}^*$ (the proof is deferred to Lemma~\ref{lem:ideal}).

We then call a transformation $G$ to be a \emph{$\nu$-code perturbation} of $\mathcal{C}^*$
if given any skeleton $\mathbf{u}$, $G(\mathbf{u})$ replaces any $c^*_i$ in it with a code $c'_i$
satisfying $\|c'_i - c^*_i\| \le \nu$.  With this definition we show that,
on an image attacked with adversarial budget $\epsilon\le 5\nu$,
our discretization $T$ will output a $\nu$-code perturbation on $\mathbf{u}$.
This leads to the following proposition whose proof is in the supplemental materials. 
\begin{prop} \label{prop:ideal}
  Assume the idealized generative model, and $\Gamma > 16\nu$ where 
  \begin{align}
    \label{eqn:ideal}
    \nu = \sigma \sqrt{\log \frac{1}{1/k - 2\gamma/\alpha}}, ~~ \gamma = \sqrt{\frac{4}{N} \log\frac{K}{\delta}},
  \end{align}
where $N$ is the number of pixels in the training dataset. Assume $r=2\nu$ in Algorithm~\ref{alg:find}.
Then for any $\epsilon\le 5\nu$,
\begin{align*}
  \textnormal{Pr}_{(\bfx,\mathbf{u},y)}[ F(T(\mathbf{z})) = y \textrm{~for any~} \|\mathbf{z} - \bfx\|
  \le \epsilon ] \ge \min_{G}\textnormal{Pr}_{(\bfx,\mathbf{u},y)}[ F(G(\mathbf{u})) = y]
\end{align*}
with probability at least $1-\delta$, where the minimum is taken over all $\nu$-code perturbation $G$.
\end{prop}

Proposition~\ref{prop:ideal} follows from the following lemma showing that our code construction method finds a set of codes close to the ground-truth codes. 

\begin{lem}
  \label{lem:ideal}
  Let $N$ denote the number of pixels in the training set. For any $\delta > 0$, if $\Gamma > 16\nu$ where $\nu$ is defined as in Proposition~\ref{prop:ideal},
  then with probability at least $1-\delta$, Algorithm~\ref{alg:find} with $r=2\nu$ outputs a set of codes $\mathcal{C} = \{c_1,\ldots, c_k\}$ such that
  $\|c_i - c^*_i\| \le \nu, \forall i$.
\end{lem}
\begin{proof}
  Let $x$ denote a pixel in the generated images. We have for any $i$, $\text{Pr}[x=c^*_i] \ge \alpha/k$,
  and for any $c$ such that $\|c-c^*_i\| \ge \nu$ for all $i$, $\Pr[x=c] \le \alpha \exp(-\nu^2/\sigma^2)$.
  By Hoeffding's inequality, with probability at least $1-\delta$, the empirical estimations satisfy
  \begin{align*}
    \widehat{\Pr}[x=c^*_i] \ge \alpha/k - \gamma,~~\widehat{\Pr}[x=c] \le \alpha \exp(-\nu^2/\sigma^2) + \gamma.
  \end{align*}
  Then $\widehat{\Pr}[x=c^*_i] > \widehat{\Pr}[x=c]$. Note that $r=2\nu$ and $\Gamma>16\nu$, so for each $c^*_i$,
  Algorithm~\ref{alg:find} picks a code from the neighborhood around $c^*_i$ of radius $\nu$ exactly once. This completes the proof.
\end{proof}

Essentially, this proposition says that we can ``reduce'' defending against $5\nu$ adversarial attacks to
defending against $\nu$-code perturbations $G$. Therefore, as long as we have a base model $F$ that is robust
to small structured perturbation (i.e., the $\nu$-code perturbation), then we can defend against
\emph{any} $5\nu$ adversarial attacks, which is a significant boost of robustness.
Encouragingly, we observed that the intuition is consistent with our experiments:
Our method gives better performance using an adversarially trained $F(\cdot)$, than a naturally trained $F$,
on structured data like MNIST.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "make"
%%% End:


==> separable-codes.tex <==
This section is structured as follows:
\begin{itemize}
\item In Section~\ref{sec:framework-and-codebook-construction} we
  present a general discretization framework which leverages a
  ``global'' codebook. We then describe separable codes and key
  properties these codes should satisfy. Finally, we present
  algorithms for constructing separable codes based on density
  estimation.

\item To provide further insights, in Section~\ref{sec:ideal} we give
  an idealized generative model of images, and formally analyze the
  effectiveness of our method for that model. Our analysis results
  demonstrate that if data indeed satisfies the well clustering
  property as dictated by separable global codes, then our method can
  provably improve adversarial robustness.

\item Finally in Section~\ref{sec:cert} we present certificates for both local and global
  robustness in practical scenarios. 
\end{itemize}

\subsection{Preprocessing Framework and Codebook Construction}
\label{sec:framework-and-codebook-construction}
At the high level, our framework is very simple and has the following two steps:
\begin{enumerate}
\item At training time, we construct a codebook $\mathcal{C}=\{c_1,c_2,\cdots,c_k\}$ for some $k$,
  where $c_i$ is in the pixel space.
  This codebook $\mathcal{C}$ is then fixed during test time.
\item Given an image $\bfx$ at test time, $T$ replaces each pixel $\bfx[i]$ with a codeword
  $c \in \mathcal{C}$ that has minimal distance to $\bfx$.
\end{enumerate}
In this work we focus on $T$ that replaces each pixel with its nearest
codeword under certain distance metric.  Many other directions are
possible and we leave those for future investigation. We now give details
about separable codes.

\noindent\textbf{Separable Codes and Construction via Density Estimation.} 
Separable codes are codes that satisfy the following two properties:
\begin{itemize}
\item {\it Separability}. Pairwise distances of codewords is large enough
  for certain distance metric.
\item {\it Representativity}. There exists a classifier $F$ that has good accuracy on the discretized data
  based on $\mathcal{C}$, as described by the framework above.
\end{itemize}
Intuitively, one may want to apply common clustering algorithms, such as $k$-means and $k$-medoids,
to find separable codes. Intriguingly, empirically we found that that such techniques do not perform well.
We therefore devise new algorithms to construct separable codes based on density estimation and greedy selection
on all the pixels $\mathcal{P}$ in the training data. This algorithm is described in Algorithm~\ref{alg:find}.
This algorithm takes as input a set of images $\mathcal{D}$, a kernel function for density estimation,
and number of codes $k$ and a distance parameter $r$. It repeats $k$ times and at each time,
first estimates the densities for all pixel values, then adds the one with highest density to the codebook,
and finally, remove all pixels within $r$ distance of the picked.

\begin{algorithm}[!htb]
  \caption{\textsc{Deriving Codes via Density Estimation}}
  \label{alg:find}
  \begin{algorithmic}[1]
    \REQUIRE A training dataset $\mathcal{D}$, parameters $r$ and $k$, a kernel function $\rho(\cdot, \cdot)$.
    \ENSURE a set of codes $\mathcal{C}=\{c_1,c_2,\cdots,c_k\}$.
    \STATE Let $\mathcal{P}$ denote all the pixels from images in $\mathcal{D}$.
    \FOR{$i=1,2,\cdots,k$}
    \STATE For each pixel value $v$, estimate its (unnormalized) density as
    $h[v] = \sum_{p \in \mathcal{P}} \rho(p, v)$.
    \STATE Set $c_i \leftarrow \arg\max_{v} h[v]$, and
    $\mathcal{P} \leftarrow \mathcal{P}-\{p\in \mathcal{P} : \|p-c_i\| \leq r \}$.
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

\textbf{\emph{Instantiation}}. There are many possible kernel functions we can use to instantiate
Algorithm~\ref{alg:find}. In this work we use the simplest choice, the identity kernel,
$\rho(p_1, p_2) = 1$ if $p_1 = p_2$ and $0$ otherwise. In that case, the density estimation at line 3
above becomes counting the frequencies of a pixel $v$ in $\mathcal{P}$.

\subsection{An Idealized Model and Its Analysis}
\label{sec:ideal}
\input{ideal}

\subsection{Certificate for the Discretization Defense}
\label{sec:cert}
Now we derive the certificates for our defense method. For a pixel $\bfx[i]$,
let $c^*(\bfx[i])$ denote its nearest code in $\mathcal{C}$, and define
\begin{align} \label{eqn:disc_deter_can}
\mathcal{C}(\bfx[i]) = \{c:  \|\bfx[i] - c\| \le \|c^*(\bfx[i]) - \bfx[i]\| + 2\epsilon \}
\end{align}
where $\epsilon$ is the adversarial budget. 
Then after perturbation bounded by $\epsilon$, the perturbed pixel has distance from $c^*(\bfx[i])$ at most $\|c^*(\bfx[i]) - \bfx[i]\|+\epsilon$, while it has distance from any $c\not\in C(\bfx[i])$ at least $\|\bfx[i] - c\|-\epsilon$. So it can only be discretized to a code in $\mathcal{C}(\bfx[i])$. 
Then all possible outcomes of the discretization after perturbation are
\begin{align} \label{eqn:disc_deter_cer1}
  \mathcal{S}(\bfx) = \{\mathbf{z} = (\mathbf{z}[1], \ldots, \mathbf{z}[d]): \mathbf{z}[i] \in \mathcal{C}(\bfx[i]) \}.
\end{align}
This then leads to the following local and global certificates.

\noindent\textbf{Local certificate.}
For a data point $(\bfx, y)$, if for any $\mathbf{z} \in \mathcal{S}(\bfx)$ we have $F(\mathbf{z}) = y$, then it is guaranteed that $\bfx$ is correctly classified by $F(T(\cdot))$ to $y$ even under the adversarial attack. 
Formally, let $\mathbb{I}_F(\bfx,y)$ be the indicator that $F(\mathbf{z}) = y$ for all $\mathbf{z} \in \mathcal{S}(\bfx)$, then
\begin{align} \label{eqn:disc_deter_cer2}
\mathbb{I}_F(\bfx,y) = \mathbb{I}[F(\mathbf{z}) = y, \forall \mathbf{z} \in \mathcal{S}(\bfx)] \le \mathbb{I}[F(T(\mathbf{z})) = y \textrm{~for any~} \|\mathbf{z} - \bfx\| \le \epsilon],
\end{align}
so $\mathbb{I}_F(\bfx,y)$ serves as a local certificate for $(\bfx, y)$.

\noindent\textbf{Global certificate.}
Define $s = \mathbb{E}_{(\bfx,y)}[\mathbb{I}_F(\bfx,y)]$. 
Then clearly, $s \le \Pr_{(\bfx,y)\sim D}[ F(T(\mathbf{z})) = y \textrm{~for any~} \|\mathbf{z} - \bfx\| \le \epsilon]$,
so $s$ serves as a lower bound for the robustness accuracy. This certificate $s$ can be estimated on a validation set of data points. Applying Hoeffding's inequality leads to the following.
\begin{prop} \label{prop:disc_deter_cer}
Let $\hat{s}$ be the frequency of $\mathcal{I}_F(\bfx,y)=1$ on a set $\mathcal{V}$ of $m$ i.i.d.\ samples from the data distribution. 
Then with probability at least $1-\delta$ over $\mathcal{V}$,
\begin{align*}
  \Pr_{(\bfx,y)\sim D}[ F(T(\mathbf{z})) = y \textrm{~for any~} \|\mathbf{z} - \bfx\| \le \epsilon]
  \ge \hat{s}_* :=\left( 1 - \sqrt{\frac{1}{2m} \log \frac{1}{\delta}} \right) \hat{s}.
\end{align*}
\end{prop}

Note that computing the certificate needs enumerating $\mathcal{S}(\bfx)$ that can be of exponential size.
However, when the pixels are well clustered, most of them are much closer to their nearest code than to the others,
and thus will not be discretized to a new code after perturbation, i.e., $|\mathcal{C}(\bfx[i])|=1$. Then $\mathcal{S}(\bfx)$ is of small size and the certificate is easy to compute.
This is indeed the case on the MNIST data, which allows us to compute the estimated certificate $\hat{s}$ in our experiments.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "make"
%%% End:

